Uplifting edges in higher order networks: spectral centralities for non-uniform hypergraphs

Spectral analysis of networks states that many structural properties of graphs, such as centrality of their nodes, are given in terms of their adjacency matrices. The natural extension of such spectral analysis to higher order networks is strongly limited by the fact that a given hypergraph could have several different adjacency hypermatrices, hence the results obtained so far are mainly restricted to the class of uniform hypergraphs, which leaves many real systems unattended. A new method for analysing non-linear eigenvector-like centrality measures of non-uniform hypergraphs is presented in this paper that could be useful for studying properties of $\mathcal{H}$-eigenvectors and $\mathcal{Z}$-eigenvectors in the non-uniform case. In order to do so, a new operation - the $\textit{uplift}$ - is introduced, incorporating auxiliary nodes in the hypergraph to allow for a uniform-like analysis. We later argue why this is a mathematically sound operation, and we furthermore use it to classify a whole family of hypergraphs with unique Perron-like $\mathcal{Z}$-eigenvectors. We supplement the theoretical analysis with several examples and numerical simulations on synthetic and real datasets.

==> numerical.tex <==

\todo[inline]{Probablemente haya que mover esta sección a ser una subsección de 3.1, y añadir a su vez una subsección de 3.2 con ejemplos numéricos de la equivalencia entre ZECs}

\missingfigure[figheight=10cm]{Varias simulaciones, que tendremos que concretar. Personalmente, considero que puede estar bien tener una tabla y dos figuras, a saber:\\
- Tabla con 10 nodos más centrales de 2 o 3 datasets reales, alguno de ellos de los de Benson, al menos uno nuevo.\\
- Figura con spearman/kendall de la diferencia de ranking entre solo uplift y HEC (con el HEC en varios niveles de uniformidad) en varios datasets (el formato de la figura habría que pensarlo), algunos sintéticos y otros reales. También comparar con la vector centrality.\\
- Figura como la anterior pero en este caso metiendo también la proyección.\\ 
Dependiendo de cómo sean las dos figuras anteriores de diferentes/interesantes, igual podríamos dejar solo la segunda.}





